NoP Generator: Package-Aware Co-Design of Chiplet Systems

Chiplet integration enables systems beyond a single die's area limit and creates opportunities for design reuse and cost reduction. Realizing these benefits requires exploring chiplet boundaries, fabrication processes, inter-chiplet networks, and packaging technologies together. We present NoP Generator, a Network-on-Package (NoP) co-design framework. Architects specify a system's functional blocks, the communication requirements between them, and the available technologies. From these inputs, the framework synthesizes a feasible package design by jointly determining chiplet boundaries, process assignments, inter-chiplet topology and routing, and the floorplan. Using the same communication requirements at each stage, the framework explores combinations of 2.5D interconnects and 3D stacking to minimize package cost or, under a cost ceiling, the total bandwidth provisioned between chiplets (installed capacity). Our seven benchmarks model chiplet-based designs used in commercial processors and accelerators. At a production volume of one million units, cost-oriented search lowers geometric mean package cost by 26.9% relative to the manual references. With each reference's package cost as the ceiling, capacity-oriented search meets the same communication requirements while reducing the geometric means of installed capacity and package cost by 16.8% and 2.1%, respectively. These results demonstrate the value of automated exploration with packaging as an active design variable. The source code and benchmarks are publicly available.

==> figures/stage2/network_primitives.tex <==
\definecolor{stageTwoInk}{HTML}{294650}\definecolor{stageTwoMuted}{HTML}{617881}\definecolor{stageTwoGuide}{HTML}{7D9199}\definecolor{stageTwoPale}{HTML}{F3F7F8}\definecolor{stageTwoFaded}{HTML}{EBEFF0}\definecolor{stageTwoBlue}{HTML}{5E99CF}\definecolor{stageTwoGreen}{HTML}{4BAD9D}\definecolor{stageTwoPink}{HTML}{EF6C7C}\definecolor{stageTwoRoute}{HTML}{1F77B4}\definecolor{stageTwoAccept}{HTML}{28776F}\definecolor{stageTwoReject}{HTML}{AA6658}\tikzset{
  sTwoScene/.style={x=1cm,y=1cm,font=\fontsize{11}{13}\selectfont},
  sTwoTitle/.style={font=\fontsize{11}{13}\selectfont,text=black},
  sTwoNote/.style={font=\fontsize{10}{11.7}\selectfont,text=black,align=center},
  sTwoPanel/.style={draw=stageTwoGuide,fill=stageTwoPale,line width=.75pt,rounded corners=2.5pt},
  sTwoCard/.style={draw=stageTwoGuide,fill=white,line width=.60pt,rounded corners=2pt},
  sTwoRegion/.style={draw=stageTwoGuide!75,fill=stageTwoPale!55,
    dash pattern=on 2.8pt off 2.0pt,line width=.65pt,rounded corners=2pt},
  sTwoChip/.style={draw=stageTwoInk,line width=.60pt,minimum size=.47cm,
    inner sep=0pt,font=\fontsize{10.6}{11}\selectfont\bfseries,text=black},
  sTwoTinyChip/.style={draw=stageTwoInk,line width=.45pt,fill=stageTwoBlue!45,
    minimum size=.13cm,inner sep=0pt},
  sTwoEdge/.style={draw=stageTwoInk!80,line width=.95pt},
  sTwoFlow/.style={draw=stageTwoInk,line width=.9pt,
    -{Latex[length=1.65mm,width=1.2mm]}},
  sTwoReject/.style={draw=stageTwoReject,line width=1.5pt,
    -{Latex[length=1.6mm,width=1.15mm]}},
  sTwoAccept/.style={draw=stageTwoAccept,line width=1.5pt,
    -{Latex[length=1.6mm,width=1.15mm]}},
  sTwoRoute/.style={draw=stageTwoRoute,line width=1.55pt,
    -{Latex[length=1.6mm,width=1.15mm]}}
}\endinput


==> figures/stage3/palette.tex <==
\definecolor{nopHBM}{HTML}{ef6c7c}\definecolor{nopIOD}{HTML}{4bad9d}\definecolor{nopXCD}{HTML}{5e99cf}\definecolor{nopInterposer}{HTML}{e0c85a}\definecolor{nopInterface}{HTML}{8E6BB5}\definecolor{nopInterfaceEdge}{HTML}{60477D}\endinput

